Unsupervised Clustered Federated Learning in Complex Multi-source Acoustic Environments

In this paper we introduce a realistic and challenging, multi-source and multi-room acoustic environment and an improved algorithm for the estimation of source-dominated microphone clusters in acoustic sensor networks. Our proposed clustering method is based on a single microphone per node and on unsupervised clustered federated learning which employs a light-weight autoencoder model. We present an improved clustering control strategy that takes into account the variability of the acoustic scene and allows the estimation of a dynamic range of clusters using reduced amounts of training data. The proposed approach is optimized using clustering-based measures and validated via a network-wide classification task.

==> Clustering EUSIPCO 2021/tex/cts_grouped.tex <==
\begin{table}
    \caption{Normalized cluster-to-source distance $\Tilde{d}_{c_x}^{s_z}$ from cluster $c_x$  to source $s_z$, averaged over 200 scenarios. Results include entire SINS apartment (4SA) and living room only (2SL).}
	\centering
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{l|ccccccccccc}
		\toprule
		  4SA    &     $c_1$     &     $c_2$     &     $c_3$     &     $c_4$     & $c_5$ & $c_6$ & $c_7$ & $c_8$ & $c_9$ & $c_{10}$ & $c_{11}$ \\ \midrule
		$s_1$ & \textbf{0.20} &     0.84      &     0.81      &     0.97      & 0.44  & 0.71  & 0.77  & 0.72  & 0.72  & 0.53   & 0.69   \\
		$s_2$ &     0.81      & \textbf{0.24} &     1.19      &     1.11      & 0.92  & 0.69  & 1.12  & 1.12  & 1.07  & 0.92   & 1.65   \\
		$s_3$ &     0.81      &     1.04      & \textbf{0.11} &     1.01      & 0.68  & 0.75  & 0.46  & 0.46  & 0.77  & 0.82   & 0.79   \\
		$s_4$ &     0.98      &     1.01      &     1.00      & \textbf{0.08} & 0.83  & 0.80  & 0.63  & 0.63  & 0.42  & 0.82   & 1.01   \\ \midrule
		
			2SL  &     $c_1$     &     $c_2$     & $c_3$ & $c_4$ & $c_5$ & $c_6$\\ \midrule
		$s_1$ & \textbf{0.08} &     0.95      & 0.37  & 0.78  & 0.48 & 0.76 \\
		$s_2$ &     0.94      & \textbf{0.09} & 0.68  & 0.28  & 0.67 & 0.30 \\
	\end{tabular}%
	}
	\label{tab:cts_grouped}
% 	\vspace{-0.4 cm}
\end{table}

==> Clustering EUSIPCO 2021/tex/cts_livingroom.tex <==
\begin{table}
    \caption{Living room only (2SL) normalized cluster-to-source distance $\Tilde{d}_{c_x}^{s_z}$ from cluster $c_x$  to source $s_z$, averaged over 200 scenarios.}
	\centering
	%				\resizebox{\textwidth}{!}{%
	\begin{tabular}{l|cccccc}
		\toprule
		      &     $c_1$     &     $c_2$     & $c_3$ & $c_4$ & $c_5$ & $c_6$\\ \midrule
		$s_1$ & \textbf{0.08} &     0.95      & 0.37  & 0.78  & 0.48 & 0.76 \\
		$s_2$ &     0.94      & \textbf{0.09} & 0.68  & 0.28  & 0.67 & 0.30 \\
	\end{tabular}%
	%				}
	\label{tab:cts_livingroom}
\end{table}

==> Clustering EUSIPCO 2021/tex/cts_sins.tex <==
\begin{table}
    \caption{Full apartment (4SA) normalized cluster-to-source distance $\Tilde{d}_{c_x}^{s_z}$ from cluster $c_x$  to source $s_z$, averaged over 200 scenarios.}
	\centering
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{l|ccccccccccc}
		\toprule
		      &     $c_1$     &     $c_2$     &     $c_3$     &     $c_4$     & $c_5$ & $c_6$ & $c_7$ & $c_8$ & $c_9$ & $c_{10}$ & $c_{11}$ \\ \midrule
		$s_1$ & \textbf{0.20} &     0.84      &     0.81      &     0.97      & 0.44  & 0.71  & 0.77  & 0.72  & 0.72  & 0.53   & 0.69   \\
		$s_2$ &     0.81      & \textbf{0.24} &     1.19      &     1.11      & 0.92  & 0.69  & 1.12  & 1.12  & 1.07  & 0.92   & 1.65   \\
		$s_3$ &     0.81      &     1.04      & \textbf{0.11} &     1.01      & 0.68  & 0.75  & 0.46  & 0.46  & 0.77  & 0.82   & 0.79   \\
		$s_4$ &     0.98      &     1.01      &     1.00      & \textbf{0.08} & 0.83  & 0.80  & 0.63  & 0.63  & 0.42  & 0.82   & 1.01   \\
	\end{tabular}%
	}
	\label{tab:cts_sins}
\end{table}

==> Clustering EUSIPCO 2021/tex/gender_acc.tex <==
\begin{table}
    \caption{Gender recognition Accuracy ($A_{cc}$) and $F_1$-score ($F_1$) of estimated clusters, without and with membership value (MV) weighting using threshold $v$, averaged over 200 scenarios. Closest-to-source (CTS) clusters or clusters with highest confidence (Confidence-based) are selected.}
	\centering
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{@{}l|lllllll@{}}
			\toprule
			Full apartment (4SA)  & no MV       & $\upsilon = 0$    & $\upsilon = 0.5$ & $\upsilon = 0.8$ & $\upsilon = 0.9$          & $\upsilon = 0.95$  \\ 
			\midrule
			CTS-based $A_{\mathrm{cc}}$ (\%)         & 83.4           & 91.5           & 93.4              & \textbf{93.7}             & 93.2             & 92.7               \\
			CTS-based $F_1$ (\%)                     & 82.4           & 90.1           & 93.1            & \textbf{93.2}             & 92.7             & 92.0               \\
			Confidence-based $A_{\mathrm{cc}}$ (\%) & 83.4           & 92.1           & \textbf{92.8}             & \textbf{92.8}             & 92.2             & 91.4               \\
			Confidence-based $F_1$ (\%)             & 82.4           & 91.3           & \textbf{92.1}             & \textbf{92.1}             & 91.3             & 90.4               \\ \midrule
			
			Living room (2SL)  \\ \midrule               
			CTS-based $A_{\mathrm{cc}}$ (\%)         & 88.1           & 98.5           & 99.0             & \textbf{99.8}             & \textbf{99.8}             & 99.5               \\
			CTS-based $F_1$ (\%)                     & 87.0           & 98.5           & 99.0             & \textbf{99.8}             & \textbf{99.8}             & 99.5               \\
			Confidence-based $A_{\mathrm{cc}}$ (\%) & 88.1           & 98.8           & 99.3             & \textbf{99.8}             & 99.3             & 99.0               \\
			Confidence-based $F_1$ (\%)             & 87.0           & 98.8           & 99.3             & \textbf{99.8}             & 99.3             & 99.0               \\ 
			

		\end{tabular}%
	}
	\label{tab:grouped_gender_acc}
% 	\vspace{-0.1 cm}
\end{table}

==> Clustering EUSIPCO 2021/tex/gender_model.tex <==
\begin{table}[t]
    \footnotesize
	\centering
	\caption{Neural network architecture of gender recognizer $e$.}
	\vspace{0.15cm}
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{@{}cccccccc@{}}
			\toprule
			\rot{Input}                      & \rot{Operator}                      & \rot{\begin{tabular}[c]{@{}c@{}}Out \\ ch.\end{tabular}} & \rot{Stride}                 & \rot{\begin{tabular}[c]{@{}c@{}}Kernel/ \\ Nodes\end{tabular}} & \rot{\begin{tabular}[c]{@{}c@{}}Batch \\ norm.\end{tabular}} & \rot{Activation}                   & \rot{Dropout} \\ \midrule
			
			
			\multicolumn{1}{c|}{501$\times$40} & \multicolumn{1}{c|}{Conv2d}  & \multicolumn{1}{c|}{32}                                       & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{5$\times$40}                                        & \multicolumn{1}{c|}{Yes}                                       & \multicolumn{1}{c|}{ReLU}    & -    \\
			
			
			 \multicolumn{1}{c|}{497$\times$32} & \multicolumn{1}{c|}{MaxPool} & \multicolumn{1}{c|}{-}                                        & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{5$\times$1}                                         & \multicolumn{1}{c|}{-}                                         & \multicolumn{1}{c|}{-}       & -       \\
			
			
			\multicolumn{1}{c|}{99$\times$32}  & \multicolumn{1}{c|}{Conv2d}  & \multicolumn{1}{c|}{64}                                       & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{3$\times$32}                                        & \multicolumn{1}{c|}{Yes}                                       & \multicolumn{1}{c|}{ReLU}    & -    \\
			
			
			 \multicolumn{1}{c|}{92$\times$64}  & \multicolumn{1}{c|}{MaxPool} & \multicolumn{1}{c|}{-}                                        & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{92$\times$1}                                        & \multicolumn{1}{c|}{-}                                         & \multicolumn{1}{c|}{-}       & -       \\ 
			
			
			\multicolumn{1}{c|}{1$\times$64}   & \multicolumn{1}{c|}{Dense}    & \multicolumn{1}{c|}{-}                                        & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{64}                                         & \multicolumn{1}{c|}{-}                                         & \multicolumn{1}{c|}{ReLU}    & 50\%       \\
			
		
% 			\multicolumn{1}{c|}{1$\times$128}  & \multicolumn{1}{c|}{Dense}    & \multicolumn{1}{c|}{-}                                        & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{64}                                          & \multicolumn{1}{c|}{-}                                         & \multicolumn{1}{c|}{ReLU}    & -       \\
			
			
			 \multicolumn{1}{c|}{1$\times$64}    & \multicolumn{1}{c|}{Dense}    & \multicolumn{1}{c|}{-}                                        & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{2}                                           & \multicolumn{1}{c|}{-}                                         & \multicolumn{1}{c|}{Softmax} & - \\      
		\end{tabular}%
	}
	\label{tab:gender}
\end{table}

==> Clustering EUSIPCO 2021/tex/livingroom_acc.tex <==
\begin{table}
	\caption{Gender recognition performance averaged over 200 scenarios of the SINS living room clustering without and with MV weighting using high-pass threshold $\upsilon$.}
	\centering
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{@{}l|lllllll@{}}
			\toprule
			& no MV & all clusters & $\upsilon = 0$ & $\upsilon = 0.5$ & $\upsilon = 0.8$ & $\upsilon = 0.9$ & $\upsilon = 0.95$  \\ \midrule
			CTS $A_{\mathrm{cc}}$ (\%)         & 82.2  & 89.2       & 93.3           & 94.0             & 94.3             & 94.8             & 94.3               \\
			CTS $F_1$ (\%)                     & 77.5  & 87.7       & 92.6           & 93.6             & 94.1             & 94.6             & 94.1               \\
			Probability $A_{\mathrm{cc}}$ (\%) & 82.2  & 89.2       & 93.0           & 94.0             & 93.8             & 93.8             & 93.3               \\
			Probability $F_1$ (\%)             & 77.5  & 87.7       & 92.4           & 93.7             & 93.6             & 93.6             & 93.0               \\ \bottomrule
		\end{tabular}%
	}
	\label{tab:livingroom_acc}
\end{table}

==> Clustering EUSIPCO 2021/tex/server.tex <==
\begin{table}[t]
\centering
\caption{Neural network architecture of autoencoder $h$.}
\vspace{0.15cm}
\label{tab:autoencoder}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c}
\hline
Layer & Input         & Operator    & \begin{tabular}[c]{@{}c@{}}Out\\ ch.\end{tabular} & Stride & \begin{tabular}[c]{@{}c@{}}Kernel/\\ Nodes\end{tabular} & Activation \\ \hline
1     & 128 x 128     & Conv2d      & 6                                                 & 1      & 5 x 5                                                   & ReLu       \\
2     & 6 x 124 x124  & MaxPool     & -                                                 & 2      & 2 x 2                                                   & -          \\
3     & 6 x 62 x 62   & Conv2d      & 16                                                & 1      & 5 x 5                                                   & ReLu       \\
4     & 16 x 58 x 58  & MaxPool     & -                                                 & 2      & 2 x 2                                                   & -          \\ \hline
5     & 16 x 29 x 29  & Dense       & -                                                 & -      & 29                                                      & ReLu       \\ \hline
6     & 16 x 29 x 29  & Unpool      & -                                                 & 2      & 2 x 2                                                   & -          \\
7     & 16 x 58 x 58  & ConvTrans2d & 6                                                 & 1      & 5 x 5                                                   & ReLu       \\
8     & 6 x 62 x 62   & Unpool      & -                                                 & 2      & 2 x 2                                                   & -          \\
9     & 6 x 124 x 124 & ConvTrans2d & 1                                                 & 1      & 5 x 5                                                   & Sigmoid   
\end{tabular}%
}
\vspace{-0.05 cm}
\end{table}

==> Clustering EUSIPCO 2021/tex/sins_T60.tex <==
\begin{table}[b]
    \vspace{-0.1 cm}
	\centering
	\caption{Room-specific floor area, simulated reverberation time ($T_{60}$) and number of randomly positioned sources and nodes.}
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{l|cccc}
		\toprule
		Room        & Floor Area   & $T_{60}$	& \# Sources & \# Nodes	  \\ \midrule
		Living room & 29.14 m$^2$  & 0.37 s	    & 2           & 24    \\
		Bedroom     & 6.51 m$^2$   & 0.27 s	    & 1           & 5    \\
		Toilet      & 1.22 m$^2$   & 0.33 s	    & 0           & 2    \\
		Corridor    & 2.86 m$^2$   & 0.42 s	    & 0           & 5    \\
		Bathroom    & 3.77 m$^2$   & 0.53 s	    & 1           & 5    \\ 
	\end{tabular}%
	}
	\label{tab:sins_t60}
	\vspace{-0.2 cm}
\end{table}


==> Clustering EUSIPCO 2021/tex/sins_acc.tex <==
\begin{table}
	\caption{Gender recognition performance averaged over 200 scenarios of the SINS apartment clustering without and with MV weighting using high-pass threshold $\upsilon$.}
	\centering
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{@{}l|lllllll@{}}
			\toprule
			& no MV & all clusters & $\upsilon = 0$ & $\upsilon = 0.5$ & $\upsilon = 0.8$ & $\upsilon = 0.9$ & $\upsilon = 0.95$  \\ \midrule
			CTS $A_{\mathrm{cc}}$ (\%)         & 80.0  & 80.6       & 94.0           & 94.6             & 94.8             & 94.6             & 94.7               \\
			CTS $F_1$ (\%)                     & 75.9  & 77.7       & 93.6           & 94.2             & 94.6             & 94.2             & 94.4               \\
			Probability $A_{\mathrm{cc}}$ (\%) & 80.0  & 80.6       & 94.1           & 94.3             & 93.4             & 93.0             & 92.9               \\
			Probability $F_1$ (\%)             & 75.9  & 77.7       & 93.8           & 94.0             & 93.1             & 92.7             & 92.6               \\ \bottomrule
		\end{tabular}%
	}
	\label{tab:sins_acc}
\end{table}

==> Clustering EUSIPCO 2021/tex/ucfl.tex <==
\begin{algorithm}[t!]
	\SetAlgoLined
	\KwIn{Pre-trained autoencoder $h$, thresholds $\varepsilon_2$ and $\varepsilon_3$, lower ($\mathit{min}_\tau$) and upper ($max_{\tau}$) communication rounds bounds}

	Freeze all parameters of $h$ except bottleneck subset $\gvec{\theta}$\\
% 	$C = \{\{1,\dots,M\}\}$\\
    \While{\text{audio buffer $!=$ empty}}{ 
    Read audio data $\gvec{D}$ of M clients \\
    Initialize cluster list $C \leftarrow \{\{1,..M\}\}$ with a single cluster element that contains all $M$ clients\\
    $\gvec\theta_c \leftarrow \gvec\theta \leftarrow$ \text{random initialization}, $\forall c \in C$\\
	$n_\mathrm{no\text{-}split}\leftarrow -1$, $\tau \leftarrow 0$\\
	\While{$\tau \leq \mathit{max}_\tau \ \text{\normalfont \textbf{and}}\  n_\mathrm{no\text{-}split} \leq \varepsilon_3$}{
		\For {$i \leftarrow 1,\dots,M$ \textbf{\textit{in parallel}}}{
			\underline{Client i does:}\\
%			$\gvec{\theta}_i^{\tau} \leftarrow \gvec{\theta}_i^{\tau-1} + \Delta \gvec{\theta}_{c(i)}^{\tau}$\\
%			$\gvec{\theta}_i^{\tau} \leftarrow \gvec{\theta}_{c(i)}^{\tau}$\\
$			\gvec{\theta}_i^{\tau} \leftarrow \gvec{\theta}_{c}^{\tau}, \ i \in c \text{ and } c \in C$\\
			$\Delta \gvec{\theta}_i^{\tau} \leftarrow \mathrm{SGD} (\gvec{\theta}_i^{\tau}, \gvec{D}_i) - \gvec{\theta}_i^{\tau}$\\
		}
		\underline{Server does:}\\
		$C' \leftarrow \{ \}$\\
		$\mathit{split} \leftarrow \mathrm{false}$\\
		\For{$c \in C$}{
			Compute $\gvec{A}_c$ and $\Delta\bar{\theta}_c, \Delta\hat{\theta}_c$ from (\ref{eq:mean_max_updates})
% 			$\Delta\bar{\theta}_c \leftarrow \left\| \frac{1}{|c|} \sum_{i \in c} \Delta \gvec{\theta}_i^{\tau} \right\| $\\
% 			$\Delta\hat{\theta}_c \leftarrow \max_{i \in c} (\| \Delta \gvec{\theta}_i^{\tau} \|)$\\
% 			$A_{i,j} \leftarrow  \frac{\langle \Delta \gvec{\theta}_i^{\tau},  \Delta \gvec{\theta}_j^{\tau} \rangle}{\|  \Delta \gvec{\theta}_i^{\tau} \| \ \|  \Delta \gvec{\theta}_j^{\tau} \|}, \ \forall i, j \in c$ \\
			
%			$\Delta \gvec{\theta}_c \leftarrow \frac{1}{|c|} \sum_{i \in c} \Delta \gvec{\theta}_i$\\
			$\text{\textbf{if}}\ \tau == 0 \text{\textbf{ then}}\ \varepsilon_1 \leftarrow \Delta\bar{\theta}_c + 0.1 \Delta\hat{\theta}_c$ \\
			\eIf{$\tau > \mathit{min}_\tau \ \text{\normalfont \textbf{and}}\  \Delta\bar{\theta}_c \leq \varepsilon_1 \ \text{\normalfont \textbf{and}}\ \frac{\Delta\bar{\theta}_c}{\Delta\hat{\theta}_c} \leq \varepsilon_2$}{
				$\{c_1, c_2\} \leftarrow \text{Bi-partitioning}(c, \gvec{A}_c)$ \\	
				$\gvec{\theta}^{\tau+1}_{c_x} \leftarrow \gvec{\theta}^{\tau}_c + \frac{1}{|c_x|}\sum_{i \in c_x} \Delta\gvec{\theta}^{\tau}_{i}, \ \forall c_x \in \{c_1, c_2\}$\\
				$\mathit{split} \leftarrow \mathrm{true}$\\
				$n_\mathrm{no\text{-}split} \leftarrow 0$\\
				$C' \leftarrow C' + \{c_1, c_2\}$\\
			}
			{
%				$\gvec{\theta}^{\tau+1} = \gvec{\theta}^{\tau} + \sum_{i=1}^{M}\frac{|\gvec{D}_{i}|}{|\gvec{D}|}\gvec{\Delta\theta}^{\tau}_{i}$\\
				$\gvec{\theta}^{\tau+1}_{c} \leftarrow\gvec{\theta}^{\tau}_c + \frac{1}{|c|}\sum_{i \in c} \Delta\gvec{\theta}^{\tau}_{i}$\\
				$C' \leftarrow C' + \{c\}$\\
			}
		}
		\If{{\normalfont\textbf{not}} $\mathit{split}$ {\normalfont \textbf{and}} $n_\mathrm{no\text{-}split} \geq 0$}{
			$n_\mathrm{no\text{-}split} \leftarrow n_\mathrm{no\text{-}split}+1$\\
		}
		$\tau \leftarrow \tau+1$ \\
		$C \leftarrow C'$ \\
	}
% 	$A_{i,j} \leftarrow  \frac{\langle \Delta \gvec{\theta}_i^{\tau-1},  \Delta \gvec{\theta}_j^{\tau-1} \rangle}{\|  \Delta \gvec{\theta}_i^{\tau-1} \| \ \|  \Delta \gvec{\theta}_j^{\tau-1} \|}, \ \forall i, j \in \{1, \dots, M\}$ \\
% 	\KwOut{$C, \gvec{A}$}
	}
	\caption{Unsupervised CFL for the estimation of source-dominated microphone clusters in ASNs.}
	\label{alg:ucfl}
\end{algorithm}


%\begin{algorithm}[t!]
%    \SetAlgoLined
%    \KwIn{Pre-trained autoencoder $h$, thresholds $\epsilon_1$, $\epsilon_2$ and $\epsilon_3$, data of $M$ clients, maximum no. of rounds $max_{\tau}$ }
%     freeze all parameters of $h$ except $\gvec{\theta}$\\
%     initialize cluster list $C = \{\{1,..M\}\}$ with a single cluster element that contains all $M$ clients\\
%     \While{\text{audio buffer $!=$ empty}}{
%        read audio $\gvec{D}$ of $M$ clients\\
%        $C' = \{\}$\\
%        \For{$c \in C$}{
%            $\gvec\theta \leftarrow$ \text{random initialization}\\
%             \While{$\tau \leq max_{\tau}$}{
%                 \For {$i \in c$}{
%                 $\gvec{\Delta \theta}^{\tau}_{i} \leftarrow SGD(h_{\gvec{\theta}}(\gvec{D}_i))$\\
%                 }
%                 $\Delta\bar{\theta} = \left\| \frac{1}{M} \sum_{i=1}^M \gvec{\Delta\theta}_i \right\| $\\
%                 $\Delta\hat{\theta} = \max_{i} (\| \gvec{\Delta\theta}_i \|)$\\
%                      \If{$\Delta\bar{\theta} \leq \epsilon_1$ \text{\&} $\Delta\hat{\theta} \geq \epsilon_2$ \text{\&} $\nabla \Delta\bar{\theta} \leq \epsilon_3$}{
%                        $a_{i,j} = \frac{\langle \gvec{\Delta\theta}_i, \gvec{\Delta\theta}_j \rangle}{\lVert \gvec{\Delta\theta}_i \rVert \lVert \gvec{\Delta\theta}_j \rVert}$, $\forall i,j \in c$\\
%                        $c_1, c_2 \leftarrow $ bi-partition ($\gvec{A}$)\\
%                        $\gvec{\theta}^{\tau+1}_{c_1} = \gvec{\theta}^{\tau} + \sum_{i\in c_1}\frac{|\gvec{D}_{i}|}{|\gvec{D}|}\gvec{\Delta\theta}^{\tau}_{i}$\\
%                        $\gvec{\theta}^{\tau+1}_{c_2} = \gvec{\theta}^{\tau} + \sum_{j\in c_{2}}\frac{|\gvec{D}_{j}|}{|\gvec{D}|}\gvec{\Delta\theta}^{\tau}_{j}$\\
%                        $C' = C' + \{c_1, c_2\}$\\
%                        exit while
%                      }
%                      \Else{
%                        $\gvec{\theta}^{\tau+1} = \gvec{\theta}^{\tau} + \sum_{i=1}^{M}\frac{|\gvec{D}_{i}|}{|\gvec{D}|}\gvec{\Delta\theta}^{\tau}_{i}$
%                        $C' = C' + \{c\}$\\
%                      }
%            }
%        }
%        $C=C'$
%     }
%     \caption{Unsupervised CFL for the estimation of source-dominated microphone clusters in ASNs}
%     \label{alg:ucfl}
%\end{algorithm}

==> Clustering EUSIPCO 2021/tex/values_grouped.tex <==
\begin{table}
	\caption{Number of simulation scenarios generating cluster $c_x$ ($N_{c_x}$) and mean number of clients in $c_x$ ($\overline{N}_{\mathrm{clients},c_x}$). Results include entire SINS apartment (4SA) and living room only (2SL).}
	\centering
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{l|ccccccccccc}
		\toprule
		                                      4SA & $c_1$   & $c_2$ & $c_3$ & $c_4$ & $c_5$ & $c_6$ & $c_7$ & $c_8$ & $c_9$ & $c_{10}$  & $c_{11}$  \\ \midrule
		$N_{c_x}$                             &  200    &  200  &  192  &  188  &  182  &  163  &  125  & 89   &  52   &  10   &    1           \\
		$\overline{N}_{\mathrm{clients},c_x}$ &  10.4   &  5.1  &  5.2  &  5.1  &  5.2  &  5.7  &  4.8  &  4.6  &  4.1  &   3.1     & 5         \\
		
				\midrule
		                                      2SL & $c_1$ & $c_2$ & $c_3$ & $c_4$ & $c_5$ & $c_6$ \\ \midrule
		$N_{c_x}$                             &  200  &  200  &  79   &  32   &   8 &   4   \\
		$\overline{N}_{\mathrm{clients},c_x}$ &  13.8   &  6.9  &   6.2   &  3.6  &   6.5 &   2.5
	\end{tabular}%
	}
%		Number of $\Tilde{d}_{c_x}$ available for computing each cluster average in Table \ref{tab:values_livingroom}, and mean number of clients in each cluster averaged over 200 simulation scenarios of the SINS apartment.
	\label{tab:values_grouped}
% 	\vspace{-0.4 cm}
\end{table}

==> Clustering EUSIPCO 2021/tex/values_livingroom.tex <==
\begin{table}
	\caption{Number of simulation scenarios generating $c_x$ ($N_{c_x}$), and mean number of clients in $c_x$ ($\overline{N}_{\mathrm{clients},c_x}$) from all 200 simulation scenarios of the SINS apartment's living room.}
	\centering
	%				\resizebox{\textwidth}{!}{%
	\begin{tabular}{l|cccccc}
		\toprule
		                                      & $c_1$ & $c_2$ & $c_3$ & $c_4$ & $c_5$ & $c_6$ \\ \midrule
		$N_{c_x}$                             &  200  &  200  &  79   &  32   &   8 &   4   \\
		$\overline{N}_{\mathrm{clients},c_x}$ &  13.8   &  6.9  &   6.2   &  3.6  &   6.5 &   2.5   \\ \bottomrule
	\end{tabular}%
	%				}
%		Number of $\Tilde{d}_{c_x}$ available for computing each cluster average in Table \ref{tab:values_livingroom}, and mean number of clients in each cluster averaged over 200 simulation scenarios of the SINS apartment's living room.
	\label{tab:values_livingroom}
\end{table}

==> Clustering EUSIPCO 2021/tex/values_sins.tex <==
\begin{table}
	\caption{Number of simulation scenarios generating $c_x$ ($N_{c_x}$), and mean number of clients in $c_x$ ($\overline{N}_{\mathrm{clients},c_x}$) from all 200 simulation scenarios of the SINS apartment.}
	\centering
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{l|ccccccccccc}
		\toprule
		                                      & $c_1$   & $c_2$ & $c_3$ & $c_4$ & $c_5$ & $c_6$ & $c_7$ & $c_8$ & $c_9$ & $c_{10}$  & $c_{10}$  \\ \midrule
		$N_{c_x}$                             &  200    &  200  &  192  &  188  &  182  &  163  &  125  & 89   &  52   &  10   &    1           \\
		$\overline{N}_{\mathrm{clients},c_x}$ &  10.4   &  5.1  &  5.2  &  5.1  &  5.2  &  5.7  &  4.8  &  4.6  &  4.1  &   3.1     & 5         \\ \bottomrule
	\end{tabular}%
	}
%		Number of $\Tilde{d}_{c_x}$ available for computing each cluster average in Table \ref{tab:values_livingroom}, and mean number of clients in each cluster averaged over 200 simulation scenarios of the SINS apartment.
	\label{tab:values_sins}
\end{table}

==> tex/cts_livingroom.tex <==
\begin{table}
    \caption{Living room only (2SL) normalized cluster-to-source distance $\Tilde{d}_{c_x}^{s_z}$ from cluster $c_x$  to source $s_z$, averaged over 200 scenarios.}
	\centering
	%				\resizebox{\textwidth}{!}{%
	\begin{tabular}{l|cccccc}
		\toprule
		      &     $c_1$     &     $c_2$     & $c_3$ & $c_4$ & $c_5$ & $c_6$\\ \midrule
		$s_1$ & \textbf{0.08} &     0.95      & 0.37  & 0.78  & 0.48 & 0.76 \\
		$s_2$ &     0.94      & \textbf{0.09} & 0.68  & 0.28  & 0.67 & 0.30 \\
	\end{tabular}%
	%				}
	\label{tab:cts_livingroom}
\end{table}

==> tex/cts_sins.tex <==
\begin{table}
    \caption{Full apartment (4SA) normalized cluster-to-source distance $\Tilde{d}_{c_x}^{s_z}$ from cluster $c_x$  to source $s_z$, averaged over 200 scenarios.}
	\centering
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{l|ccccccccccc}
		\toprule
		      &     $c_1$     &     $c_2$     &     $c_3$     &     $c_4$     & $c_5$ & $c_6$ & $c_7$ & $c_8$ & $c_9$ & $c_{10}$ & $c_{11}$ \\ \midrule
		$s_1$ & \textbf{0.20} &     0.84      &     0.81      &     0.97      & 0.44  & 0.71  & 0.77  & 0.72  & 0.72  & 0.53   & 0.69   \\
		$s_2$ &     0.81      & \textbf{0.24} &     1.19      &     1.11      & 0.92  & 0.69  & 1.12  & 1.12  & 1.07  & 0.92   & 1.65   \\
		$s_3$ &     0.81      &     1.04      & \textbf{0.11} &     1.01      & 0.68  & 0.75  & 0.46  & 0.46  & 0.77  & 0.82   & 0.79   \\
		$s_4$ &     0.98      &     1.01      &     1.00      & \textbf{0.08} & 0.83  & 0.80  & 0.63  & 0.63  & 0.42  & 0.82   & 1.01   \\
	\end{tabular}%
	}
	\label{tab:cts_sins}
\end{table}

==> tex/gender_model.tex <==
\begin{table}[t]
    \footnotesize
	\centering
	\caption{Neural network architecture of gender recognizer $e$.}
	\vspace{0.15cm}
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{@{}cccccccc@{}}
			\toprule
			\rot{Input}                      & \rot{Operator}                      & \rot{\begin{tabular}[c]{@{}c@{}}Out \\ ch.\end{tabular}} & \rot{Stride}                 & \rot{\begin{tabular}[c]{@{}c@{}}Kernel/ \\ Nodes\end{tabular}} & \rot{\begin{tabular}[c]{@{}c@{}}Batch \\ norm.\end{tabular}} & \rot{Activation}                   & \rot{Dropout} \\ \midrule
			
			
			\multicolumn{1}{c|}{501$\times$40} & \multicolumn{1}{c|}{Conv2d}  & \multicolumn{1}{c|}{32}                                       & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{5$\times$40}                                        & \multicolumn{1}{c|}{Yes}                                       & \multicolumn{1}{c|}{ReLU}    & -    \\
			
			
			 \multicolumn{1}{c|}{497$\times$32} & \multicolumn{1}{c|}{MaxPool} & \multicolumn{1}{c|}{-}                                        & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{5$\times$1}                                         & \multicolumn{1}{c|}{-}                                         & \multicolumn{1}{c|}{-}       & -       \\
			
			
			\multicolumn{1}{c|}{99$\times$32}  & \multicolumn{1}{c|}{Conv2d}  & \multicolumn{1}{c|}{64}                                       & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{3$\times$32}                                        & \multicolumn{1}{c|}{Yes}                                       & \multicolumn{1}{c|}{ReLU}    & -    \\
			
			
			 \multicolumn{1}{c|}{92$\times$64}  & \multicolumn{1}{c|}{MaxPool} & \multicolumn{1}{c|}{-}                                        & \multicolumn{1}{c|}{1} & \multicolumn{1}{c|}{92$\times$1}                                        & \multicolumn{1}{c|}{-}                                         & \multicolumn{1}{c|}{-}       & -       \\ 
			
			
			\multicolumn{1}{c|}{1$\times$64}   & \multicolumn{1}{c|}{Dense}    & \multicolumn{1}{c|}{-}                                        & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{64}                                         & \multicolumn{1}{c|}{-}                                         & \multicolumn{1}{c|}{ReLU}    & 50\%       \\
			
		
% 			\multicolumn{1}{c|}{1$\times$128}  & \multicolumn{1}{c|}{Dense}    & \multicolumn{1}{c|}{-}                                        & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{64}                                          & \multicolumn{1}{c|}{-}                                         & \multicolumn{1}{c|}{ReLU}    & -       \\
			
			
			 \multicolumn{1}{c|}{1$\times$64}    & \multicolumn{1}{c|}{Dense}    & \multicolumn{1}{c|}{-}                                        & \multicolumn{1}{c|}{-} & \multicolumn{1}{c|}{2}                                           & \multicolumn{1}{c|}{-}                                         & \multicolumn{1}{c|}{Softmax} & - \\      
		\end{tabular}%
	}
	\label{tab:gender}
\end{table}

==> tex/livingroom_acc.tex <==
\begin{table}
	\caption{Gender recognition performance averaged over 200 scenarios of the SINS living room clustering without and with MV weighting using high-pass threshold $\upsilon$.}
	\centering
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{@{}l|lllllll@{}}
			\toprule
			& no MV & all clusters & $\upsilon = 0$ & $\upsilon = 0.5$ & $\upsilon = 0.8$ & $\upsilon = 0.9$ & $\upsilon = 0.95$  \\ \midrule
			CTS $A_{\mathrm{cc}}$ (\%)         & 82.2  & 89.2       & 93.3           & 94.0             & 94.3             & 94.8             & 94.3               \\
			CTS $F_1$ (\%)                     & 77.5  & 87.7       & 92.6           & 93.6             & 94.1             & 94.6             & 94.1               \\
			Probability $A_{\mathrm{cc}}$ (\%) & 82.2  & 89.2       & 93.0           & 94.0             & 93.8             & 93.8             & 93.3               \\
			Probability $F_1$ (\%)             & 77.5  & 87.7       & 92.4           & 93.7             & 93.6             & 93.6             & 93.0               \\ \bottomrule
		\end{tabular}%
	}
	\label{tab:livingroom_acc}
\end{table}

==> tex/sins_acc.tex <==
\begin{table}
	\caption{Gender recognition performance averaged over 200 scenarios of the SINS apartment clustering without and with MV weighting using high-pass threshold $\upsilon$.}
	\centering
	\resizebox{\columnwidth}{!}{%
		\begin{tabular}{@{}l|lllllll@{}}
			\toprule
			& no MV & all clusters & $\upsilon = 0$ & $\upsilon = 0.5$ & $\upsilon = 0.8$ & $\upsilon = 0.9$ & $\upsilon = 0.95$  \\ \midrule
			CTS $A_{\mathrm{cc}}$ (\%)         & 80.0  & 80.6       & 94.0           & 94.6             & 94.8             & 94.6             & 94.7               \\
			CTS $F_1$ (\%)                     & 75.9  & 77.7       & 93.6           & 94.2             & 94.6             & 94.2             & 94.4               \\
			Probability $A_{\mathrm{cc}}$ (\%) & 80.0  & 80.6       & 94.1           & 94.3             & 93.4             & 93.0             & 92.9               \\
			Probability $F_1$ (\%)             & 75.9  & 77.7       & 93.8           & 94.0             & 93.1             & 92.7             & 92.6               \\ \bottomrule
		\end{tabular}%
	}
	\label{tab:sins_acc}
\end{table}

==> tex/values_livingroom.tex <==
\begin{table}
	\caption{Number of simulation scenarios generating $c_x$ ($N_{c_x}$), and mean number of clients in $c_x$ ($\overline{N}_{\mathrm{clients},c_x}$) from all 200 simulation scenarios of the SINS apartment's living room.}
	\centering
	%				\resizebox{\textwidth}{!}{%
	\begin{tabular}{l|cccccc}
		\toprule
		                                      & $c_1$ & $c_2$ & $c_3$ & $c_4$ & $c_5$ & $c_6$ \\ \midrule
		$N_{c_x}$                             &  200  &  200  &  79   &  32   &   8 &   4   \\
		$\overline{N}_{\mathrm{clients},c_x}$ &  13.8   &  6.9  &   6.2   &  3.6  &   6.5 &   2.5   \\ \bottomrule
	\end{tabular}%
	%				}
%		Number of $\Tilde{d}_{c_x}$ available for computing each cluster average in Table \ref{tab:values_livingroom}, and mean number of clients in each cluster averaged over 200 simulation scenarios of the SINS apartment's living room.
	\label{tab:values_livingroom}
\end{table}

==> tex/values_sins.tex <==
\begin{table}
	\caption{Number of simulation scenarios generating $c_x$ ($N_{c_x}$), and mean number of clients in $c_x$ ($\overline{N}_{\mathrm{clients},c_x}$) from all 200 simulation scenarios of the SINS apartment.}
	\centering
	\resizebox{\columnwidth}{!}{%
	\begin{tabular}{l|ccccccccccc}
		\toprule
		                                      & $c_1$   & $c_2$ & $c_3$ & $c_4$ & $c_5$ & $c_6$ & $c_7$ & $c_8$ & $c_9$ & $c_{10}$  & $c_{10}$  \\ \midrule
		$N_{c_x}$                             &  200    &  200  &  192  &  188  &  182  &  163  &  125  & 89   &  52   &  10   &    1           \\
		$\overline{N}_{\mathrm{clients},c_x}$ &  10.4   &  5.1  &  5.2  &  5.1  &  5.2  &  5.7  &  4.8  &  4.6  &  4.1  &   3.1     & 5         \\ \bottomrule
	\end{tabular}%
	}
%		Number of $\Tilde{d}_{c_x}$ available for computing each cluster average in Table \ref{tab:values_livingroom}, and mean number of clients in each cluster averaged over 200 simulation scenarios of the SINS apartment.
	\label{tab:values_sins}
\end{table}
